Operads and bialgebras of multi-indices, and Novikov algebras

Noncommutative multi-indices are noncommutative monomials in a $\mathbb{N}$-indexed family of indeterminates. We define on them a $\mathbb{Z}$-graded operadic structure, with the help of a shifting derivation. Multi-indices of degree 0 are called populated: they form a suboperad, isomorphic to the operad of Novikov algebras. This operadic structure, and the relation between pre-Lie and Novikov algebras, induces two bialgebraic structure in cointeraction on commutative multi-indices. We show how to combinatorially embed this double bialgebra into the Connes-Kreimer Hopf algebra of rooted trees, with its two coproducts based, firstly on cuts, secondly, on contraction of edges, and how this embedding can be characterized by a Dyson-Schwinger equation. We also study the unique polynomial invariant compatible with the two bialgebraic structures on multi-indices and use to describe the antipode for the first coproduct.

==> posets.tex <==
\newcommand{\ptroisun}{\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.5cm,y=0.5cm]
\clip(-0.5,-0.1) rectangle (0.5,0.7);
\draw [line width=0.5pt] (0.,0.5)-- (-0.3,0.);
\draw [line width=0.5pt] (0.,0.5)-- (0.3,0.);
\begin{scriptsize}
\draw [fill=black] (-0.3,0.) circle (1pt);
\draw [fill=black] (0.,0.5) circle (1pt);
\draw [fill=black] (0.3,0.) circle (1pt);
\end{scriptsize}
\end{tikzpicture}}

\newcommand{\pquatreun}{\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.5cm,y=0.5cm]
\clip(-0.5,-0.1) rectangle (0.5,0.7);
\draw [line width=0.5pt] (0.,0.5)-- (-0.3,0.);
\draw [line width=0.5pt] (0.,0.5)-- (0.3,0.);
\draw [line width=0.5pt] (0.,0.5)-- (0.,0.);
\begin{scriptsize}
\draw [fill=black] (-0.3,0.) circle (1.0pt);
\draw [fill=black] (0.,0.5) circle (1.0pt);
\draw [fill=black] (0.3,0.) circle (1.0pt);
\draw [fill=black] (0.,0.) circle (1.0pt);
\end{scriptsize}
\end{tikzpicture}}
\newcommand{\pquatredeux}{\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.5cm,y=0.5cm]
\clip(-0.5,-0.1) rectangle (0.5,1.2);
\draw [line width=0.5pt] (0.,1.)-- (-0.3,0.5);
\draw [line width=0.5pt] (0.,1.)-- (0.3,0.5);
\draw [line width=0.5pt] (-0.3,0.5)-- (-0.3,0.);
\begin{scriptsize}
\draw [fill=black] (-0.3,0.5) circle (1.0pt);
\draw [fill=black] (0.,1.) circle (1.0pt);
\draw [fill=black] (0.3,0.5) circle (1.0pt);
\draw [fill=black] (-0.3,0.) circle (1.0pt);
\end{scriptsize}
\end{tikzpicture}}
\newcommand{\pquatretrois}{\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.5cm,y=0.5cm]
\clip(-0.5,-0.1) rectangle (0.5,1.2);
\draw [line width=0.5pt] (0.,1.)-- (-0.3,0.5);
\draw [line width=0.5pt] (0.,1.)-- (0.3,0.5);
\draw [line width=0.5pt] (0.3,0.5)-- (0.3,0.);
\begin{scriptsize}
\draw [fill=black] (-0.3,0.5) circle (1.0pt);
\draw [fill=black] (0.,1.) circle (1.0pt);
\draw [fill=black] (0.3,0.5) circle (1.0pt);
\draw [fill=black] (0.3,0.) circle (1.0pt);
\end{scriptsize}
\end{tikzpicture}}
\newcommand{\pquatrequatre}{\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.5cm,y=0.5cm]
\clip(-0.5,-0.1) rectangle (0.5,1.7);
\draw [line width=0.5pt] (0.,1.)-- (0.,0.5);
\draw [line width=0.5pt] (0.,0.5)-- (0.3,0.);
\draw [line width=0.5pt] (0.,0.5)-- (-0.3,0.);
\begin{scriptsize}
\draw [fill=black] (0.,1.) circle (1.0pt);
\draw [fill=black] (0.,0.5) circle (1.0pt);
\draw [fill=black] (-0.3,0.) circle (1.0pt);
\draw [fill=black] (0.3,0.) circle (1.0pt);
\end{scriptsize}
\end{tikzpicture}}
\newcommand{\pquatrecinq}{\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.5cm,y=0.5cm]
\clip(-0.5,-0.1) rectangle (0.5,0.7);
\draw [line width=0.5pt] (-0.3,0.)-- (-0.3,0.5);
\draw [line width=0.5pt] (0.3,0.)-- (0.3,0.5);
\draw [line width=0.5pt] (-0.3,0.)-- (0.3,0.5);
\begin{scriptsize}
\draw [fill=black] (-0.3,0.) circle (1pt);
\draw [fill=black] (0.3,0.) circle (1pt);
\draw [fill=black] (-0.3,0.5) circle (1pt);
\draw [fill=black] (0.3,0.5) circle (1pt);
\end{scriptsize}
\end{tikzpicture}}
\newcommand{\pquatresix}{\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.5cm,y=0.5cm]
\clip(-0.5,-0.1) rectangle (0.5,0.7);
\draw [line width=0.5pt] (-0.3,0.)-- (-0.3,0.5);
\draw [line width=0.5pt] (0.3,0.)-- (0.3,0.5);
\draw [line width=0.5pt] (0.3,0.)-- (-0.3,0.5);
\begin{scriptsize}
\draw [fill=black] (-0.3,0.) circle (1pt);
\draw [fill=black] (0.3,0.) circle (1pt);
\draw [fill=black] (-0.3,0.5) circle (1pt);
\draw [fill=black] (0.3,0.5) circle (1pt);
\end{scriptsize}
\end{tikzpicture}}
\newcommand{\pquatresept}{\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.5cm,y=0.5cm]
\clip(-0.5,-0.1) rectangle (0.5,0.7);
\draw [line width=0.5pt] (-0.3,0.)-- (-0.3,0.5);
\draw [line width=0.5pt] (0.3,0.)-- (0.3,0.5);
\draw [line width=0.5pt] (0.3,0.)-- (-0.3,0.5);
\draw [line width=0.5pt] (-0.3,0.)-- (0.3,0.5);
\begin{scriptsize}
\draw [fill=black] (-0.3,0.) circle (1pt);
\draw [fill=black] (0.3,0.) circle (1pt);
\draw [fill=black] (-0.3,0.5) circle (1pt);
\draw [fill=black] (0.3,0.5) circle (1pt);
\end{scriptsize}
\end{tikzpicture}}
\newcommand{\pquatrehuit}{\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.5cm,y=0.5cm]
\clip(-0.5,-0.1) rectangle (0.5,1.2);
\draw [line width=0.5pt] (0.,1.)-- (-0.3,0.5);
\draw [line width=0.5pt] (0.,1.)-- (0.3,0.5);
\draw [line width=0.5pt] (-0.3,0.5)-- (0.,0.);
\draw [line width=0.5pt] (0.3,0.5)-- (0.,0.);
\begin{scriptsize}
\draw [fill=black] (-0.3,0.5) circle (1.0pt);
\draw [fill=black] (0.,1.) circle (1.0pt);
\draw [fill=black] (0.3,0.5) circle (1.0pt);
\draw [fill=black] (0.,0.) circle (1.0pt);
\end{scriptsize}
\end{tikzpicture}}

\newcommand{\pdtroisun}[3]{\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.5cm,y=0.5cm]
\clip(-0.7,-0.1) rectangle (0.7,1.2);
\draw [line width=0.5pt] (0.,0.5)-- (-0.3,0.);
\draw [line width=0.5pt] (0.,0.5)-- (0.3,0.);
\begin{scriptsize}
\draw [fill=black] (-0.3,0.) circle (1pt);
\draw [fill=black] (0.,0.5) circle (1pt);
\draw [fill=black] (0.3,0.) circle (1pt);
\end{scriptsize}
\draw(0.,0.8) node {\tiny #1};
\draw(-0.6,0.1) node {\tiny #2};
\draw(0.6,0.1) node {\tiny #3};
\end{tikzpicture}}



